Neutral Pion Electroproduction in the Resonance Region at High $Q^2$

The process $ep \to e^{\prime}p^{\prime}\pi^0$ has been measured at $Q^2$ = 6.4 and 7.7 GeV/c$^2$)$^2$ in Jefferson Lab's Hall C. Unpolarized differential cross sections are reported in the virtual photon-proton center of mass frame considering the process $\gamma^{\ast}p \to p^{\prime}\pi^0$. Various details relating to the background subtractions, radiative corrections and systematic errors are discussed. The usefulness of the data with regard to the measurement of the electromagnetic properties of the well known $\Delta(1232)$ resonance is covered in detail. Specifically considered are the electromagnetic and scalar-magnetic ratios $R_{EM}$ and $R_{SM}$ along with the magnetic transition form factor $G_M^{\ast}$. It is found that the rapid fall off of the $\Delta(1232)$ contribution continues into this region of momentum transfer and that other resonances

==> xntblsapp.tex <==
\appendix*
\section{Tables of Differential Cross Sections}
The measured differential cross sections mentioned throughout the text are listed here.  The author
can be contacted for an electronic version of these data points.  
\newpage
\begin{widetext}
\begin{center}
 \begin{longtable}{ccccccccc}
  \caption{\label{T:xntabl}Differential cross sections for the small SOS spectrometer angle.} \\
  \hline
  \hline
$Q^2$ &$\epsilon$ &$W$ &$\cos{\cm{\theta}}$ &$\cm{\phi}$ &$d\sigma^{\gamma^{\ast}}$ &$\sigma_{stat}$ &$\sigma_{norm}$ &$\sigma_{sys}$ \\
(GeV$^2$) &none &(GeV) &none &(rad) &(nb/Sr) &(nb/Sr) &(nb/Sr) &(nb/Sr) \\
  \hline \\[0.05cm]
  \endfirsthead
$Q^2$ &$\epsilon$ &$W$ &$\cos{\cm{\theta}}$ &$\cm{\phi}$ &$d\sigma^{\gamma^{\ast}}$ &$\sigma_{stat}$ &$\sigma_{norm}$ &$\sigma_{sys}$ \\
(GeV$^2$) &none &(GeV) &none &(rad) &(nb/Sr) &(nb/Sr) &(nb/Sr) &(nb/Sr) \\
  \hline \\[0.05cm]
  \endhead
6.564 &0.4523 &1.112 &-0.9 &-2.827 &5.1456 &3.8602 &0.29671 &0.0022301 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &-1.571 &7.3159 &5.1838 &0.42185 &0.00092151 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &-0.9425 &4.721 &3.3702 &0.27223 &0.0081633 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &-0.3142 &6.7928 &6.7933 &0.39169 &0.0002199 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &0.3142 &4.2895 &4.2898 &0.24734 &0.0023096 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &0.9425 &2.2098 &2.2099 &0.12742 &0.0043183 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &1.571 &2.2215 &2.2216 &0.1281 &0.0026498 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.9 &2.199 &2.6294 &2.6295 &0.15162 &0.0038613 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &-2.827 &9.0972 &6.964 &0.52457 &8.987e-06 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &-1.571 &5.3862 &3.8094 &0.31059 &0.0012255 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &-0.9425 &3.0943 &3.0944 &0.17843 &0.00088908 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &-0.3142 &18.853 &10.933 &1.0871 &0.0018922 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &0.3142 &10.064 &10.064 &0.5803 &0.0037097 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &0.9425 &3.1474 &3.1475 &0.18149 &0.0027893 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &1.571 &4.9941 &3.6308 &0.28798 &0.00041656 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.7 &2.199 &5.2545 &3.7235 &0.30299 &0.0012938 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &-2.827 &6.9861 &5.0843 &0.40284 &0.00013218 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &-2.199 &5.2735 &3.7522 &0.30408 &0.0015351 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &-1.571 &15.133 &9.2937 &0.87261 &0.00040333 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &-0.9425 &3.8679 &3.8681 &0.22303 &0.00025298 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &-0.3142 &9.3756 &6.6308 &0.54062 &0.0015795 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &0.3142 &25.968 &13.199 &1.4974 &0.0024584 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &0.9425 &6.8284 &3.9439 &0.39375 &0.00024808 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &1.571 &3.7445 &2.6479 &0.21592 &0.00048817 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &2.199 &10.019 &5.0939 &0.5777 &0.00022567 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.5 &2.827 &2.2994 &2.2995 &0.13259 &0.00096042 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &-2.827 &2.1049 &2.105 &0.12138 &0.00022043 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &-2.199 &2.1232 &2.1233 &0.12243 &0.00066444 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &-1.571 &5.0376 &3.6624 &0.29048 &0.00023 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &-0.9425 &11.234 &5.759 &0.6478 &0.0015196 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &-0.3142 &57.944 &37.256 &3.3412 &0.023004 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &0.3142 &60.951 &37.025 &3.5146 &0.015764 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &1.571 &4.2344 &3.0186 &0.24417 &1.9907e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &2.199 &8.5962 &5.8576 &0.49568 &0.00070534 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.3 &2.827 &10.139 &4.5686 &0.58464 &0.00037001 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &-2.827 &21.981 &18.924 &1.2675 &0.00044294 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &-2.199 &15.078 &6.4268 &0.86942 &0.00046145 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &-0.9425 &7.9584 &5.628 &0.45891 &0.00028018 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &-0.3142 &12.381 &7.4374 &0.71391 &0.0060386 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &0.3142 &38.655 &14.038 &2.2289 &0.012986 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &0.9425 &32.695 &11.241 &1.8853 &0.00096376 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &1.571 &5.07 &3.6534 &0.29235 &0.00045379 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &2.199 &16.158 &6.9458 &0.93172 &2.4304e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &-0.1 &2.827 &17.923 &7.5007 &1.0335 &0.00013431 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &-2.827 &12.606 &5.3866 &0.72692 &0.00038193 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &-2.199 &33.452 &11.706 &1.929 &0.00028722 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &-1.571 &10.135 &5.1739 &0.58443 &4.7344e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &-0.9425 &16.65 &7.618 &0.96009 &0.001648 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &-0.3142 &14.395 &7.2267 &0.83003 &0.00039035 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &0.3142 &11.853 &8.3824 &0.68346 &0.002947 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &0.9425 &13.464 &6.896 &0.77635 &0.0033774 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &1.571 &7.8324 &4.5961 &0.45164 &0.00061512 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &2.199 &13.884 &7.775 &0.8006 &0.00046377 \\[0.05cm]
6.564 &0.4523 &1.112 &0.1 &2.827 &13.592 &7.157 &0.78377 &0.0008163 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &-2.827 &14.904 &9.1123 &0.85938 &0.00045971 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &-2.199 &22.41 &9.1013 &1.2922 &0.00045136 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &-1.571 &10.256 &8.349 &0.59136 &0.00027807 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &-0.9425 &22.719 &9.5587 &1.3101 &0.00095757 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &-0.3142 &27.617 &11.673 &1.5925 &0.0018643 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &0.3142 &20.849 &9.6313 &1.2022 &0.0013521 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &0.9425 &18.643 &7.0854 &1.075 &0.00021287 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &1.571 &14.325 &7.9453 &0.82605 &0.00039282 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &2.199 &27.426 &10.06 &1.5815 &0.00060565 \\[0.05cm]
6.564 &0.4523 &1.112 &0.3 &2.827 &22.962 &10.861 &1.324 &0.0005877 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &-2.827 &28.368 &18.777 &1.6358 &0.0004772 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &-2.199 &24.278 &8.3812 &1.3999 &0.0001755 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &-1.571 &32.625 &22.218 &1.8813 &0.003919 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &-0.9425 &37.605 &17.136 &2.1684 &0.0028012 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &-0.3142 &35.366 &12.874 &2.0393 &0.00030649 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &0.3142 &24.391 &11.036 &1.4064 &0.00054765 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &0.9425 &14.804 &6.7183 &0.85365 &0.00037035 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &1.571 &43.139 &17.449 &2.4875 &0.0012527 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &2.199 &15.212 &6.482 &0.87716 &1.7868e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &0.5 &2.827 &32.087 &18.393 &1.8502 &0.00052026 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &-2.827 &5.4717 &4.0181 &0.31551 &0.0014365 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &-2.199 &38.809 &12.614 &2.2378 &5.7393e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &-1.571 &23.678 &10.283 &1.3654 &0.00098633 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &-0.9425 &12.714 &7.4858 &0.73313 &0.0003508 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &-0.3142 &14.735 &7.4909 &0.84964 &8.5562e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &0.3142 &40.752 &12.842 &2.3499 &0.0024313 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &0.9425 &13.33 &6.0632 &0.76863 &0.00046927 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &1.571 &24.513 &9.0204 &1.4135 &0.00025205 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &2.199 &32.706 &15.462 &1.8859 &9.436e-05 \\[0.05cm]
6.564 &0.4523 &1.112 &0.7 &2.827 &63.927 &31.212 &3.6862 &0.0051859 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &-2.827 &30.989 &10.439 &1.7869 &0.00033136 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &-2.199 &29.378 &9.8405 &1.694 &0.00052095 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &-1.571 &27.13 &10.884 &1.5644 &0.00057601 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &-0.9425 &29.978 &13.043 &1.7286 &0.0014522 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &-0.3142 &17.01 &6.9561 &0.98082 &0.00012777 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &0.3142 &22.102 &8.4554 &1.2745 &0.0003135 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &0.9425 &22.467 &8.2086 &1.2955 &0.00082809 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &1.571 &8.625 &4.3782 &0.49734 &0.001486 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &2.199 &66.815 &24.061 &3.8527 &0.00072457 \\[0.05cm]
6.564 &0.4523 &1.112 &0.9 &2.827 &41.745 &14.142 &2.4071 &0.0010978 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &-2.827 &18.145 &6.9597 &1.0463 &0.0017944 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &-2.199 &6.0778 &3.5869 &0.35046 &0.00249 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &-1.571 &26.717 &9.6402 &1.5406 &0.0049899 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &-0.9425 &1.9034 &1.9035 &0.10976 &0.0022291 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &-0.3142 &19.498 &11.898 &1.1243 &0.0046318 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &0.3142 &11.033 &6.3937 &0.6362 &0.0030675 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &0.9425 &9.2862 &5.3746 &0.53547 &0.0024866 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &1.571 &18.096 &7.0113 &1.0435 &0.0017757 \\[0.05cm]
6.5 &0.45 &1.152 &-0.9 &2.199 &17.026 &7.1308 &0.98179 &0.00083069 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &-2.827 &35.433 &15.445 &2.0432 &0.0014057 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &-2.199 &13.571 &5.5982 &0.78253 &0.0025068 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &-1.571 &13.082 &5.8924 &0.75437 &0.00065575 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &-0.9425 &12.134 &5.4747 &0.69971 &0.00075663 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &-0.3142 &6.9187 &5.0035 &0.39895 &0.0024212 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &0.3142 &21.501 &9.7855 &1.2398 &0.0020319 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &0.9425 &10.937 &5.5517 &0.63064 &0.00021486 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &1.571 &15.875 &6.1564 &0.9154 &0.00083043 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &2.199 &11.743 &4.8013 &0.67715 &0.00080767 \\[0.05cm]
6.5 &0.45 &1.152 &-0.7 &2.827 &1.9803 &1.9804 &0.11419 &0.001676 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &-2.827 &8.0384 &3.6342 &0.46352 &0.00031068 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &-2.199 &26.937 &8.9194 &1.5533 &1.098e-05 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &-1.571 &16.887 &6.0553 &0.97376 &0.00089984 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &-0.9425 &23.01 &7.8875 &1.3268 &0.0012879 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &-0.3142 &10.717 &6.1916 &0.61795 &0.0017522 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &0.3142 &46.007 &15.642 &2.6529 &0.0017078 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &0.9425 &20.201 &6.8789 &1.1648 &0.00118 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &1.571 &15.294 &5.646 &0.88189 &0.00017736 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &2.199 &23.898 &8.7182 &1.378 &1.9861e-05 \\[0.05cm]
6.5 &0.45 &1.152 &-0.5 &2.827 &12.896 &10.352 &0.74359 &0.00024213 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &-2.827 &23.739 &6.7723 &1.3689 &0.00028304 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &-2.199 &12.511 &4.8968 &0.72144 &0.0007588 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &-1.571 &20.064 &6.5212 &1.157 &0.0021651 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &-0.9425 &18.918 &6.8887 &1.0909 &0.0018553 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &-0.3142 &27.414 &8.8345 &1.5808 &0.014441 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &0.3142 &42.518 &12.234 &2.4517 &0.017976 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &0.9425 &20.871 &7.1753 &1.2035 &0.00092685 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &1.571 &17.69 &6.9128 &1.02 &0.0041457 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &2.199 &18.642 &6.8938 &1.0749 &0.00027403 \\[0.05cm]
6.5 &0.45 &1.152 &-0.3 &2.827 &19.092 &7.0354 &1.1009 &6.3843e-06 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &-2.827 &14.411 &5.2958 &0.83096 &0.0014044 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &-2.199 &20.98 &6.6856 &1.2098 &0.00026931 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &-1.571 &16.894 &6.0924 &0.97413 &0.00079208 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &-0.9425 &20.26 &7.446 &1.1682 &0.00087771 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &-0.3142 &36.521 &11.339 &2.1059 &0.0076459 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &0.3142 &11.814 &5.3081 &0.68124 &0.0084097 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &0.9425 &3.8207 &2.7026 &0.22031 &0.0016472 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &1.571 &14.694 &5.3006 &0.84727 &0.0017377 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &2.199 &24.899 &8.0518 &1.4357 &0.00012292 \\[0.05cm]
6.5 &0.45 &1.152 &-0.1 &2.827 &30.757 &8.5402 &1.7736 &0.0001201 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &-2.827 &13.383 &5.2515 &0.77168 &0.00017631 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &-2.199 &41.686 &11.285 &2.4037 &0.00017777 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &-1.571 &14.612 &5.2148 &0.84254 &0.00082403 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &-0.9425 &9.2767 &5.3739 &0.53492 &0.00049922 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &-0.3142 &15.571 &7.9025 &0.89788 &0.00088619 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &0.3142 &18.741 &7.3384 &1.0807 &0.0046192 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &0.9425 &29.882 &8.5191 &1.7231 &0.0017976 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &1.571 &34.162 &10.313 &1.9699 &0.00017074 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &2.199 &22.97 &6.6448 &1.3245 &0.0012701 \\[0.05cm]
6.5 &0.45 &1.152 &0.1 &2.827 &43.99 &12.208 &2.5366 &0.0010365 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &-2.827 &26.326 &9.7949 &1.518 &0.000462 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &-2.199 &20.305 &7.196 &1.1708 &0.00085251 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &-1.571 &19.847 &8.7072 &1.1444 &0.00065724 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &-0.9425 &24.887 &8.6559 &1.435 &0.00049459 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &-0.3142 &37.103 &11.063 &2.1395 &0.0023242 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &0.3142 &37.843 &11.874 &2.1821 &0.0017162 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &0.9425 &27.256 &8.5396 &1.5716 &0.0010433 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &1.571 &24.902 &7.4202 &1.4359 &6.5783e-05 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &2.199 &29.977 &9.1231 &1.7285 &0.0004178 \\[0.05cm]
6.5 &0.45 &1.152 &0.3 &2.827 &26.785 &10.582 &1.5445 &0.00309 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &-2.827 &17.809 &7.7468 &1.0269 &0.00026925 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &-2.199 &59.77 &15.197 &3.4465 &0.00045901 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &-1.571 &54.885 &13.22 &3.1648 &7.9631e-05 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &-0.9425 &34.496 &8.9942 &1.9892 &0.00096374 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &-0.3142 &39.983 &12.232 &2.3055 &0.00043831 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &0.3142 &55.739 &14.814 &3.2141 &0.0011752 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &0.9425 &16.555 &5.5869 &0.95462 &0.00034137 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &1.571 &52.215 &13.614 &3.0109 &0.00028911 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &2.199 &35.357 &9.897 &2.0388 &0.00083541 \\[0.05cm]
6.5 &0.45 &1.152 &0.5 &2.827 &36.966 &14.893 &2.1316 &0.00086477 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &-2.827 &49.923 &13.337 &2.8787 &0.00092059 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &-2.199 &41.519 &10.262 &2.3941 &0.0037733 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &-1.571 &33.824 &9.7252 &1.9504 &0.0012732 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &-0.9425 &22.934 &6.5803 &1.3225 &0.00092187 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &-0.3142 &36.184 &10.087 &2.0865 &0.00054938 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &0.3142 &26.19 &8.226 &1.5102 &0.00035521 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &0.9425 &39.571 &11.679 &2.2818 &0.00050139 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &1.571 &46.772 &12.078 &2.697 &0.0021948 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &2.199 &39.04 &10.677 &2.2512 &0.00013605 \\[0.05cm]
6.5 &0.45 &1.152 &0.7 &2.827 &60.45 &14.574 &3.4857 &0.00088343 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &-2.827 &40.017 &11.149 &2.3075 &0.00081449 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &-2.199 &48.039 &11.803 &2.7701 &0.0009598 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &-1.571 &45.695 &9.9498 &2.6349 &0.0013404 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &-0.9425 &76.266 &20.674 &4.3977 &0.0010198 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &-0.3142 &54.504 &16.521 &3.1429 &5.0556e-05 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &0.3142 &32.686 &9.1808 &1.8848 &0.00035991 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &0.9425 &60.824 &14.202 &3.5073 &6.831e-05 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &1.571 &40.541 &9.8438 &2.3377 &0.0002841 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &2.199 &43.4 &9.7059 &2.5025 &2.1757e-05 \\[0.05cm]
6.5 &0.45 &1.152 &0.9 &2.827 &53.709 &19.513 &3.097 &0.0015346 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &-2.827 &11.047 &4.6631 &0.63698 &0.0017573 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &-2.199 &24.648 &6.9704 &1.4213 &0.0013357 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &-1.571 &45.288 &16.74 &2.6115 &0.0023814 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &-0.9425 &42.322 &9.851 &2.4404 &0.0015309 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &-0.3142 &22.343 &9.9233 &1.2884 &0.001362 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &0.3142 &22.652 &9.4033 &1.3062 &0.0019144 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &0.9425 &18.813 &6.1967 &1.0848 &0.0017846 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &1.571 &24.661 &7.3622 &1.422 &1.2567e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &2.199 &24.424 &6.8611 &1.4083 &0.0002261 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.9 &2.827 &31.82 &11.863 &1.8348 &0.0029783 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &-2.827 &28.185 &9.2268 &1.6252 &0.001725 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &-2.199 &35.426 &9.3556 &2.0428 &0.0019855 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &-1.571 &29.784 &8.1188 &1.7174 &0.0026646 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &-0.9425 &55.417 &12.542 &3.1955 &0.0083037 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &-0.3142 &48.56 &14.913 &2.8001 &0.003259 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &0.3142 &50.004 &15.059 &2.8833 &0.0053559 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &0.9425 &26.731 &7.896 &1.5414 &3.3419e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &1.571 &29.246 &7.8775 &1.6864 &0.0010023 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &2.199 &17.781 &6.3649 &1.0253 &0.0019437 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.7 &2.827 &31.563 &8.7715 &1.82 &0.00079598 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &-2.827 &28.746 &8.2293 &1.6576 &0.00084156 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &-2.199 &39.526 &11.852 &2.2792 &0.0001476 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &-1.571 &43.261 &17.984 &2.4945 &0.0023327 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &-0.9425 &53.978 &11.313 &3.1125 &0.0011343 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &-0.3142 &51.655 &13.837 &2.9786 &0.0010873 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &0.3142 &54.787 &14.796 &3.1592 &0.0019867 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &0.9425 &54.459 &11.06 &3.1403 &0.001325 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &1.571 &37.297 &13.053 &2.1507 &0.0010589 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &2.199 &29.37 &10.165 &1.6935 &0.00065385 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.5 &2.827 &27.495 &6.1536 &1.5854 &0.0010455 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &-2.827 &43.185 &11.579 &2.4901 &0.001904 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &-2.199 &38.691 &10.822 &2.231 &0.0024219 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &-1.571 &50.054 &14.629 &2.8862 &0.0020117 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &-0.9425 &63.103 &12.934 &3.6387 &0.0026457 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &-0.3142 &77.045 &14.807 &4.4427 &0.018186 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &0.3142 &74.528 &15.104 &4.2975 &0.014635 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &0.9425 &27.35 &7.5086 &1.5771 &0.00083163 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &1.571 &89.809 &21.563 &5.1786 &0.001246 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &2.199 &58.367 &17.32 &3.3656 &0.0025915 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.3 &2.827 &37.457 &8.4084 &2.1599 &4.4495e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &-2.827 &35.32 &7.8296 &2.0367 &0.0002033 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &-2.199 &59.419 &14.124 &3.4263 &5.4025e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &-1.571 &34.666 &9.183 &1.9989 &0.00044981 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &-0.9425 &51.695 &12.076 &2.9809 &0.0015011 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &-0.3142 &95.15 &26.268 &5.4866 &0.010962 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &0.3142 &56.694 &12.538 &3.2691 &0.0077864 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &0.9425 &68.652 &21.746 &3.9586 &0.0043344 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &1.571 &35.836 &9.3193 &2.0664 &0.0013248 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &2.199 &43.109 &10.151 &2.4858 &3.3311e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &-0.1 &2.827 &46.285 &10.656 &2.6689 &0.0014317 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &-2.827 &79.955 &17.092 &4.6104 &7.4407e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &-2.199 &43.811 &9.7757 &2.5263 &0.0010392 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &-1.571 &45.899 &11.973 &2.6467 &0.001071 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &-0.9425 &55.775 &11.93 &3.2161 &0.0014437 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &-0.3142 &62.749 &14.164 &3.6183 &0.0017714 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &0.3142 &37.805 &10.843 &2.18 &0.0020403 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &0.9425 &29.956 &7.9284 &1.7273 &0.00034143 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &1.571 &57.834 &19.107 &3.3349 &0.0056951 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &2.199 &33.906 &7.7846 &1.9551 &0.0030093 \\[0.05cm]
6.432 &0.4478 &1.192 &0.1 &2.827 &41.235 &10.208 &2.3778 &0.001641 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &-2.827 &47.77 &11.179 &2.7546 &0.00086585 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &-2.199 &69.988 &15.938 &4.0357 &0.0012414 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &-1.571 &62.945 &20.301 &3.6296 &0.00065579 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &-0.9425 &80.802 &19.506 &4.6593 &0.00032797 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &-0.3142 &68.292 &15.698 &3.9379 &0.0010534 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &0.3142 &52.328 &15.615 &3.0174 &0.0010422 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &0.9425 &33.607 &8.0047 &1.9378 &0.00045524 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &1.571 &71.83 &14.919 &4.1419 &0.0012859 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &2.199 &44.478 &10.993 &2.5647 &5.7678e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &0.3 &2.827 &66.182 &14.344 &3.8163 &0.0022443 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &-2.827 &94.764 &16.202 &5.4644 &0.00040157 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &-2.199 &56.739 &11.954 &3.2717 &0.00066717 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &-1.571 &49.39 &11.362 &2.8479 &0.00095012 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &-0.9425 &85.094 &19.058 &4.9067 &0.00093055 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &-0.3142 &56.275 &12.409 &3.245 &0.0013954 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &0.3142 &67.789 &15.117 &3.9089 &0.00060798 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &0.9425 &63.116 &12.198 &3.6394 &0.0011835 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &1.571 &71.326 &12.892 &4.1129 &0.0002749 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &2.199 &58.193 &12.186 &3.3556 &7.5024e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &0.5 &2.827 &80.451 &15.107 &4.639 &0.00085522 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &-2.827 &51.448 &11.836 &2.9667 &0.0011189 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &-2.199 &78.941 &17.349 &4.552 &0.00022782 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &-1.571 &103.82 &18.255 &5.9868 &0.0005465 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &-0.9425 &79.718 &14.855 &4.5968 &0.0010483 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &-0.3142 &49.725 &9.8744 &2.8673 &0.0016501 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &0.3142 &57.82 &10.855 &3.3341 &2.2313e-05 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &0.9425 &78.133 &12.584 &4.5054 &0.0016997 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &1.571 &78.355 &13.502 &4.5181 &0.0015644 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &2.199 &66.477 &11.946 &3.8332 &0.00063365 \\[0.05cm]
6.432 &0.4478 &1.192 &0.7 &2.827 &59.141 &12.569 &3.4102 &0.00036994 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &-2.827 &63.212 &13.286 &3.645 &0.00010471 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &-2.199 &54.003 &9.4179 &3.114 &0.0007965 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &-1.571 &93.327 &13.419 &5.3815 &0.0007686 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &-0.9425 &69.687 &16.513 &4.0183 &0.0023462 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &-0.3142 &61.987 &14.489 &3.5744 &0.0010639 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &0.3142 &63.185 &12.025 &3.6434 &0.00070092 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &0.9425 &81.207 &14.881 &4.6826 &0.0014375 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &1.571 &80.916 &20.473 &4.6659 &0.0013868 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &2.199 &51.885 &10.638 &2.9918 &0.00082569 \\[0.05cm]
6.432 &0.4478 &1.192 &0.9 &2.827 &84.188 &15.339 &4.8545 &0.00022091 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &-2.827 &15.312 &4.605 &0.88292 &0.001517 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &-2.199 &25.252 &6.1039 &1.4561 &0.0027001 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &-1.571 &37.53 &7.9536 &2.1641 &0.00067805 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &-0.9425 &34.347 &10.427 &1.9805 &0.0026516 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &-0.3142 &30.797 &8.9147 &1.7758 &0.0031805 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &0.3142 &28.524 &9.3511 &1.6447 &0.0020863 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &0.9425 &27.62 &6.444 &1.5926 &7.031e-05 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &1.571 &33.082 &7.2796 &1.9076 &0.0017309 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &2.199 &34.401 &7.0448 &1.9837 &0.0022476 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.9 &2.827 &21.963 &7.6983 &1.2664 &0.00037634 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &-2.827 &27.57 &7.4844 &1.5898 &0.00032556 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &-2.199 &36.404 &8.0381 &2.0992 &0.0015433 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &-1.571 &51.64 &10.012 &2.9777 &0.003794 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &-0.9425 &57.63 &10.962 &3.3231 &0.0014462 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &-0.3142 &65.346 &14.304 &3.768 &0.0065457 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &0.3142 &65.697 &16.863 &3.7883 &0.0016551 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &0.9425 &50.514 &13.263 &2.9128 &0.0034051 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &1.571 &48.571 &12.223 &2.8008 &0.0038736 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &2.199 &36.219 &7.6593 &2.0885 &0.0011033 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.7 &2.827 &38.04 &9.7684 &2.1935 &0.00066715 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &-2.827 &43.092 &10.536 &2.4848 &0.0017767 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &-2.199 &48.155 &10.411 &2.7768 &0.0028237 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &-1.571 &70.797 &12.665 &4.0824 &0.00080946 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &-0.9425 &63.329 &11.1 &3.6517 &5.541e-06 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &-0.3142 &75.061 &15.262 &4.3282 &0.0018716 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &0.3142 &59.978 &13.635 &3.4585 &0.0018035 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &0.9425 &72.405 &15.696 &4.1751 &0.0026738 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &1.571 &74.959 &18.7 &4.3223 &0.0012664 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &2.199 &59.181 &13.319 &3.4126 &0.0011206 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.5 &2.827 &48.721 &10.649 &2.8094 &0.002804 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &-2.827 &52.596 &11.09 &3.0328 &0.0011402 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &-2.199 &81.241 &14.102 &4.6846 &0.0015378 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &-1.571 &62.403 &13.687 &3.5983 &0.0005429 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &-0.9425 &73.443 &12.615 &4.2349 &0.0020155 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &-0.3142 &71.866 &12.812 &4.144 &0.0061375 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &0.3142 &71.594 &13.009 &4.1283 &0.0074144 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &0.9425 &108.86 &25.662 &6.2773 &0.00089949 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &1.571 &79.938 &13.518 &4.6094 &0.0057605 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &2.199 &68.875 &16.57 &3.9716 &0.0046297 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.3 &2.827 &60.028 &11.536 &3.4614 &0.0041212 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &-2.827 &64.765 &9.5423 &3.7346 &0.0024374 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &-2.199 &84.171 &17.293 &4.8535 &0.0036526 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &-1.571 &112.77 &25.293 &6.5026 &0.0014334 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &-0.9425 &86.905 &15.323 &5.0112 &0.0010962 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &-0.3142 &106.02 &16.89 &6.1134 &0.0097303 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &0.3142 &101.15 &22.191 &5.8329 &0.0038596 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &0.9425 &86.11 &21.226 &4.9653 &0.0021845 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &1.571 &55.976 &12.382 &3.2277 &0.0011441 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &2.199 &47.448 &9.7851 &2.736 &5.9008e-06 \\[0.05cm]
6.36 &0.4458 &1.232 &-0.1 &2.827 &49.069 &8.5789 &2.8294 &0.0014101 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &-2.827 &53.531 &10.393 &3.0868 &9.4144e-05 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &-2.199 &83.063 &15.758 &4.7896 &0.00078709 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &-1.571 &63.644 &14.934 &3.6699 &0.001439 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &-0.9425 &74.696 &21.837 &4.3072 &0.0015447 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &-0.3142 &69.573 &12.845 &4.0118 &0.0059268 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &0.3142 &51.227 &10.521 &2.9539 &0.00067524 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &0.9425 &64.016 &12.158 &3.6913 &0.0013558 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &1.571 &80.044 &20.181 &4.6155 &0.0016172 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &2.199 &81.437 &14.52 &4.6959 &0.0024828 \\[0.05cm]
6.36 &0.4458 &1.232 &0.1 &2.827 &79.154 &11.915 &4.5642 &0.00092908 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &-2.827 &71.664 &13.363 &4.1324 &0.00079553 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &-2.199 &89.505 &17.766 &5.1611 &0.0016149 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &-1.571 &128.9 &42.053 &7.4327 &5.3625e-06 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &-0.9425 &75.91 &14.39 &4.3772 &0.00050794 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &-0.3142 &53.933 &11.162 &3.1099 &0.00080985 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &0.3142 &66.883 &13.521 &3.8566 &0.0020579 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &0.9425 &86.768 &14.784 &5.0033 &0.00058984 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &1.571 &114.6 &31.162 &6.6083 &0.00050502 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &2.199 &85.347 &16.087 &4.9214 &0.00066831 \\[0.05cm]
6.36 &0.4458 &1.232 &0.3 &2.827 &79.942 &15.359 &4.6097 &0.0026732 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &-2.827 &92.591 &14.692 &5.3391 &0.0015941 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &-2.199 &89.586 &14.677 &5.1658 &0.00018426 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &-1.571 &89.307 &20.186 &5.1497 &0.00085133 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &-0.9425 &87.486 &15.438 &5.0447 &0.0011996 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &-0.3142 &71.488 &12.958 &4.1222 &0.0039979 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &0.3142 &83.917 &13.874 &4.8389 &0.0003316 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &0.9425 &93.863 &15.557 &5.4124 &0.00066131 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &1.571 &92.108 &17.973 &5.3112 &0.00071987 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &2.199 &97.534 &15.702 &5.6241 &0.00099951 \\[0.05cm]
6.36 &0.4458 &1.232 &0.5 &2.827 &100.04 &15.473 &5.7689 &0.0010367 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &-2.827 &68.52 &12.571 &3.9511 &0.00058737 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &-2.199 &74.222 &13.504 &4.2798 &0.00019433 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &-1.571 &91.863 &20.175 &5.2971 &0.00078697 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &-0.9425 &95.628 &15.097 &5.5142 &0.00028129 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &-0.3142 &81.033 &14.335 &4.6726 &0.0013743 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &0.3142 &61.255 &11.24 &3.5322 &0.00093099 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &0.9425 &67.752 &12.165 &3.9068 &0.0018143 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &1.571 &95.528 &18.751 &5.5084 &0.0017806 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &2.199 &75.469 &12.255 &4.3518 &0.00046249 \\[0.05cm]
6.36 &0.4458 &1.232 &0.7 &2.827 &69.796 &12.272 &4.0247 &0.00038327 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &-2.827 &57.881 &10.417 &3.3376 &5.5006e-05 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &-2.199 &67.481 &9.7999 &3.8911 &0.00076371 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &-1.571 &85.337 &15.327 &4.9208 &0.0012856 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &-0.9425 &90.126 &15.779 &5.1969 &0.0016165 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &-0.3142 &67.788 &11.106 &3.9088 &0.0010264 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &0.3142 &66.124 &11.274 &3.8129 &0.00022832 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &0.9425 &57.317 &10.094 &3.3051 &0.0016569 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &1.571 &73.394 &10.526 &4.2321 &0.00021915 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &2.199 &71.379 &13.647 &4.1159 &0.00057609 \\[0.05cm]
6.36 &0.4458 &1.232 &0.9 &2.827 &77.137 &16.682 &4.4479 &0.0013301 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &-2.827 &17.862 &4.3654 &1.03 &0.0020241 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &-2.199 &26.296 &5.6051 &1.5163 &0.0019327 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &-1.571 &39.285 &8.8843 &2.2653 &0.0017382 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &-0.9425 &26.024 &5.8255 &1.5006 &0.00036234 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &-0.3142 &20.5 &6.3519 &1.1821 &0.0018713 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &0.3142 &27.889 &9.8767 &1.6081 &0.0012021 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &0.9425 &20.553 &4.8753 &1.1851 &0.001044 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &1.571 &28.054 &7.8183 &1.6177 &0.0014454 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &2.199 &10.549 &3.1536 &0.60828 &0.0017805 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.9 &2.827 &15.511 &3.8518 &0.8944 &0.0015084 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &-2.827 &15.477 &5.085 &0.89247 &0.00095308 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &-2.199 &23.56 &5.6609 &1.3585 &0.001779 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &-1.571 &48.35 &9.6118 &2.788 &0.00023927 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &-0.9425 &47.201 &8.3991 &2.7217 &0.00026839 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &-0.3142 &37.918 &10.736 &2.1864 &0.0029986 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &0.3142 &57.389 &14.27 &3.3092 &0.003198 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &0.9425 &38.487 &8.5191 &2.2193 &0.0038085 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &1.571 &41.263 &7.9373 &2.3793 &0.0043012 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &2.199 &28.847 &6.3335 &1.6634 &0.00092686 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.7 &2.827 &14.348 &3.5442 &0.82733 &0.00034734 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &-2.827 &34.786 &5.9809 &2.0059 &0.00026079 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &-2.199 &38.021 &7.0756 &2.1924 &0.0027052 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &-1.571 &101.93 &16.193 &5.8778 &0.00098498 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &-0.9425 &70.413 &17.189 &4.0602 &0.0036787 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &-0.3142 &63.539 &12.789 &3.6639 &0.0031812 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &0.3142 &69.845 &13.713 &4.0274 &0.0019379 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &0.9425 &77.803 &11.332 &4.4863 &0.0032345 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &1.571 &57.645 &10.645 &3.324 &0.0034227 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &2.199 &27.338 &6.2147 &1.5764 &0.0025916 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.5 &2.827 &27.715 &5.1889 &1.5981 &0.00030037 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &-2.827 &38.613 &6.2438 &2.2265 &0.0026174 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &-2.199 &44.887 &9.0571 &2.5883 &0.00046712 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &-1.571 &79.797 &17.239 &4.6013 &0.0048101 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &-0.9425 &62.699 &11.299 &3.6154 &0.0035716 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &-0.3142 &77.152 &13.005 &4.4488 &0.0044233 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &0.3142 &59.584 &11.729 &3.4358 &0.011622 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &0.9425 &78.648 &12.409 &4.5351 &0.0013722 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &1.571 &82.807 &17.684 &4.7749 &0.0026722 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &2.199 &71.452 &13.002 &4.1201 &0.00037482 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.3 &2.827 &37.881 &6.0099 &2.1843 &0.0025311 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &-2.827 &63.136 &9.3848 &3.6406 &0.0017405 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &-2.199 &66.818 &14.204 &3.8529 &0.00079563 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &-1.571 &83.161 &25.551 &4.7953 &0.0049019 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &-0.9425 &72.155 &14.495 &4.1607 &1.1454e-05 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &-0.3142 &112.91 &17.04 &6.5108 &0.0078861 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &0.3142 &80.132 &12.539 &4.6207 &0.012298 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &0.9425 &82.633 &22.583 &4.7648 &0.0011514 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &1.571 &110.17 &44.79 &6.3526 &0.016987 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &2.199 &72.493 &14.603 &4.1801 &0.0017879 \\[0.05cm]
6.288 &0.4434 &1.272 &-0.1 &2.827 &32.709 &5.9622 &1.8861 &0.001 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &-2.827 &62.071 &9.3363 &3.5792 &9.999e-05 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &-2.199 &53.081 &13.199 &3.0608 &0.0011983 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &-1.571 &66.484 &26.953 &3.8337 &0.0038983 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &-0.9425 &43.638 &10.98 &2.5163 &0.0012127 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &-0.3142 &88.367 &20.863 &5.0955 &0.0022072 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &0.3142 &80.702 &15.058 &4.6535 &0.0011381 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &0.9425 &84.933 &22.331 &4.8975 &0.00022908 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &1.571 &99.45 &30.373 &5.7346 &0.013716 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &2.199 &50.086 &11.069 &2.8881 &0.0038067 \\[0.05cm]
6.288 &0.4434 &1.272 &0.1 &2.827 &50.608 &7.469 &2.9182 &0.00066077 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &-2.827 &57.829 &9.4832 &3.3346 &0.00035005 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &-2.199 &71.627 &16.657 &4.1302 &0.00073316 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &-1.571 &80.008 &36.594 &4.6135 &0.0081551 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &-0.9425 &100.13 &18.55 &5.7739 &0.00085984 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &-0.3142 &61.108 &11.37 &3.5236 &0.00020759 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &0.3142 &62.299 &10.644 &3.5923 &0.0015516 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &0.9425 &85.45 &15.525 &4.9273 &0.0047196 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &1.571 &58.464 &23.093 &3.3712 &0.0090907 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &2.199 &89.772 &15.556 &5.1765 &0.0029753 \\[0.05cm]
6.288 &0.4434 &1.272 &0.3 &2.827 &59.394 &8.5765 &3.4248 &0.00075794 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &-2.827 &62.478 &11.928 &3.6026 &0.00067135 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &-2.199 &85.667 &16.371 &4.9398 &0.0012174 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &-1.571 &89.213 &24.659 &5.1443 &0.0091419 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &-0.9425 &127.5 &20.504 &7.3522 &0.0015404 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &-0.3142 &70.453 &13.341 &4.0625 &0.0031454 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &0.3142 &54.221 &10.614 &3.1265 &7.597e-05 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &0.9425 &68.866 &13.808 &3.971 &0.0025189 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &1.571 &101.21 &27.93 &5.8363 &0.00039421 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &2.199 &56.366 &13.01 &3.2502 &0.0014987 \\[0.05cm]
6.288 &0.4434 &1.272 &0.5 &2.827 &45.303 &8.1424 &2.6123 &2.4001e-05 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &-2.827 &55.441 &10.55 &3.1969 &0.00010367 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &-2.199 &74.162 &13.796 &4.2764 &0.00035785 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &-1.571 &88.116 &25.949 &5.081 &0.00098667 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &-0.9425 &58.92 &12.798 &3.3975 &0.0012494 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &-0.3142 &32.655 &8.1072 &1.883 &0.0011939 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &0.3142 &100.14 &20.594 &5.7745 &0.0028999 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &0.9425 &55.57 &11.281 &3.2043 &0.00077688 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &1.571 &94.388 &29.991 &5.4427 &0.0055059 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &2.199 &53.468 &9.9044 &3.0831 &0.00081286 \\[0.05cm]
6.288 &0.4434 &1.272 &0.7 &2.827 &60.184 &11.534 &3.4704 &0.0017275 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &-2.827 &45.413 &11.935 &2.6186 &0.0026551 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &-2.199 &78.923 &14.442 &4.5509 &0.00080164 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &-1.571 &68.132 &12.781 &3.9287 &0.00033059 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &-0.9425 &81.846 &15.797 &4.7195 &0.0007442 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &-0.3142 &36.74 &8.0495 &2.1186 &0.0028121 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &0.3142 &68.843 &13.773 &3.9697 &1.1416e-05 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &0.9425 &64.778 &10.265 &3.7353 &0.00073718 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &1.571 &58.402 &9.3582 &3.3676 &0.00097404 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &2.199 &68.837 &10.233 &3.9694 &0.0018396 \\[0.05cm]
6.288 &0.4434 &1.272 &0.9 &2.827 &44.959 &9.0113 &2.5925 &0.0041438 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &-2.827 &22.092 &6.1225 &1.2739 &0.00064087 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &-2.199 &26.309 &6.598 &1.517 &0.0038275 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &-1.571 &13.843 &4.0981 &0.79822 &0.0021118 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &-0.9425 &18.905 &4.6508 &1.0901 &0.0014662 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &-0.3142 &9.7009 &4.2151 &0.55938 &0.0032457 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &0.3142 &13.506 &5.1767 &0.77879 &0.0041159 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &0.9425 &26.343 &7.697 &1.519 &0.0016104 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &1.571 &17.465 &4.2123 &1.0071 &0.0022664 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &2.199 &19.893 &6.9237 &1.1471 &0.0013353 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.9 &2.827 &18.828 &4.1756 &1.0857 &0.0037768 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &-2.827 &24.289 &5.1997 &1.4006 &0.00038549 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &-2.199 &17.024 &4.6724 &0.98168 &0.0019656 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &-1.571 &31.323 &9.5501 &1.8061 &0.0049943 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &-0.9425 &43.769 &8.1768 &2.5238 &0.0028492 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &-0.3142 &31.729 &9.1608 &1.8296 &0.0015942 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &0.3142 &37.244 &9.4202 &2.1476 &0.002736 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &0.9425 &41.41 &8.5809 &2.3878 &0.0020117 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &1.571 &36.316 &7.535 &2.0941 &0.0015338 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &2.199 &26.152 &7.1373 &1.508 &0.0013004 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.7 &2.827 &24.613 &5.6119 &1.4192 &0.00020145 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &-2.827 &42.224 &6.3488 &2.4347 &0.0023581 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &-2.199 &35.169 &8.1947 &2.0279 &9.9461e-05 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &-1.571 &54.217 &13.496 &3.1263 &0.00039987 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &-0.9425 &73.6 &11.606 &4.244 &0.003327 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &-0.3142 &67.631 &20.647 &3.8998 &0.0065659 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &0.3142 &56.442 &11.501 &3.2546 &0.003 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &0.9425 &58.732 &10.697 &3.3866 &0.0028821 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &1.571 &57.765 &17.432 &3.3309 &0.0031817 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &2.199 &30.455 &6.9368 &1.7561 &0.0033316 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.5 &2.827 &26.118 &4.6402 &1.506 &0.0018558 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &-2.827 &30.157 &5.3377 &1.7389 &0.001479 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &-2.199 &61.649 &10.949 &3.5549 &0.0010369 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &-1.571 &40.573 &15.437 &2.3395 &0.00067139 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &-0.9425 &70.334 &13.924 &4.0556 &6.0195e-05 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &-0.3142 &70.964 &16.785 &4.092 &0.0022087 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &0.3142 &69.051 &16.771 &3.9817 &0.010021 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &0.9425 &48.628 &10.714 &2.804 &0.0033021 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &1.571 &48.912 &16.454 &2.8204 &0.0046566 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &2.199 &46.677 &9.3636 &2.6916 &0.0021328 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.3 &2.827 &45.213 &6.6512 &2.6071 &0.0013777 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &-2.827 &48.245 &7.5442 &2.7819 &0.0024892 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &-2.199 &53.21 &15.278 &3.0682 &0.00037206 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &-0.9425 &81.474 &18.357 &4.698 &0.0049676 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &-0.3142 &66.836 &11.196 &3.8539 &0.013021 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &0.3142 &72.724 &11.91 &4.1934 &0.01089 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &0.9425 &55.117 &13.665 &3.1782 &0.0010518 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &2.199 &61.574 &14.677 &3.5505 &0.0032287 \\[0.05cm]
6.212 &0.4411 &1.312 &-0.1 &2.827 &47.464 &9.1527 &2.7369 &0.0012146 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &-2.827 &58.144 &13.869 &3.3528 &0.00031254 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &-2.199 &40.609 &12.302 &2.3417 &0.0026161 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &-0.9425 &63.686 &17.464 &3.6723 &0.0046476 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &-0.3142 &80.119 &12.777 &4.6199 &0.0026031 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &0.3142 &76.712 &12.803 &4.4234 &0.0013351 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &0.9425 &69.302 &21.048 &3.9961 &0.00011976 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &2.199 &76.756 &17.422 &4.4259 &0.0010479 \\[0.05cm]
6.212 &0.4411 &1.312 &0.1 &2.827 &41.144 &7.0438 &2.3725 &0.00043057 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &-2.827 &34.918 &7.1395 &2.0135 &0.0023171 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &-2.199 &68.882 &22.264 &3.9719 &0.0015446 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &-1.571 &701.32 &542.84 &40.44 &0.10864 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &-0.9425 &64.894 &18.437 &3.742 &0.00037813 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &-0.3142 &48.66 &9.9505 &2.8059 &0.0012379 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &0.3142 &62.635 &9.8494 &3.6117 &0.00031635 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &0.9425 &61.357 &22.612 &3.538 &0.002907 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &1.571 &440.51 &199.36 &25.401 &0.040725 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &2.199 &53.725 &15.067 &3.098 &0.00078191 \\[0.05cm]
6.212 &0.4411 &1.312 &0.3 &2.827 &51.882 &8.2552 &2.9916 &0.001264 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &-2.827 &68.419 &11.954 &3.9452 &9.0561e-06 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &-2.199 &50.91 &16.86 &2.9356 &0.0011619 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &-0.9425 &67.367 &18.053 &3.8846 &0.0028328 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &-0.3142 &74.501 &11.552 &4.2959 &0.00011422 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &0.3142 &62.503 &11.399 &3.6041 &8.825e-05 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &0.9425 &98.142 &21.918 &5.6591 &0.0024758 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &2.199 &73.625 &17.299 &4.2454 &0.00070443 \\[0.05cm]
6.212 &0.4411 &1.312 &0.5 &2.827 &51.248 &9.2744 &2.9551 &0.00059057 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &-2.827 &51.129 &9.0324 &2.9483 &0.0022247 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &-2.199 &86.081 &17.185 &4.9637 &0.00043576 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &-1.571 &167.18 &51.03 &9.6401 &0.0054201 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &-0.9425 &42.069 &12.137 &2.4258 &0.0015007 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &-0.3142 &45.342 &9.3753 &2.6146 &0.0020303 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &0.3142 &55.263 &9.1647 &3.1866 &0.0021157 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &0.9425 &92.016 &22.862 &5.3059 &0.0014702 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &1.571 &51.298 &18.703 &2.958 &0.0025673 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &2.199 &85.439 &18.214 &4.9267 &0.00098577 \\[0.05cm]
6.212 &0.4411 &1.312 &0.7 &2.827 &48.768 &9.4658 &2.8121 &0.00281 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &-2.827 &75.204 &12.689 &4.3365 &0.0010756 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &-2.199 &73.252 &13.277 &4.2239 &0.00012054 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &-1.571 &56.078 &10.137 &3.2336 &8.4007e-05 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &-0.9425 &51.926 &11.666 &2.9942 &0.0016308 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &-0.3142 &49.776 &9.1364 &2.8702 &0.00038724 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &0.3142 &60.162 &9.9891 &3.4691 &0.0022023 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &0.9425 &56.182 &9.944 &3.2396 &0.0002606 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &1.571 &60.876 &9.744 &3.5103 &0.0024472 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &2.199 &48.701 &8.4289 &2.8082 &0.0028085 \\[0.05cm]
6.212 &0.4411 &1.312 &0.9 &2.827 &91.543 &14.662 &5.2786 &0.00045347 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &-2.827 &16.9 &4.116 &0.97449 &0.0013485 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &-2.199 &16.474 &3.9983 &0.94994 &0.0016662 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &-1.571 &17.563 &3.9571 &1.0127 &0.00095739 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &-0.9425 &11.962 &3.3637 &0.68975 &0.00067235 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &-0.3142 &6.2004 &2.9192 &0.35753 &0.0018939 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &0.3142 &12.375 &4.5811 &0.7136 &0.0019949 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &0.9425 &30.205 &7.258 &1.7417 &0.003687 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &1.571 &19.695 &4.3013 &1.1357 &0.00111 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &2.199 &19.978 &4.0317 &1.152 &0.0011619 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.9 &2.827 &23.071 &4.6789 &1.3303 &0.0023663 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &-2.827 &26.438 &6.972 &1.5245 &0.0008259 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &-2.199 &19.29 &5.149 &1.1123 &0.0031291 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &-1.571 &36.309 &10.428 &2.0937 &0.00011443 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &-0.9425 &26.536 &6.2464 &1.5302 &0.0035206 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &-0.3142 &29.802 &8.1555 &1.7184 &0.00164 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &0.3142 &26.99 &8.0375 &1.5563 &0.0020909 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &0.9425 &28.787 &6.2777 &1.6599 &0.0037673 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &1.571 &51.391 &12.914 &2.9633 &0.0021992 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &2.199 &9.4572 &3.0493 &0.54533 &0.0032143 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.7 &2.827 &35.462 &7.4235 &2.0448 &0.0031742 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &-2.827 &33.998 &5.3225 &1.9604 &0.001537 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &-2.199 &44.391 &11.194 &2.5597 &0.0015143 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &-1.571 &59.872 &24.501 &3.4524 &0.0015665 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &-0.9425 &69.019 &12.09 &3.9798 &0.0029591 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &-0.3142 &57.025 &10.892 &3.2882 &0.0050064 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &0.3142 &43.507 &9.2729 &2.5087 &0.0039238 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &0.9425 &88.362 &18.304 &5.0952 &0.00029216 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &1.571 &41.326 &12.235 &2.3829 &0.00093083 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &2.199 &35.675 &9.854 &2.0571 &0.00077604 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.5 &2.827 &17.545 &4.0789 &1.0117 &0.001441 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &-2.827 &35.617 &6.3857 &2.0538 &0.00014756 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &-2.199 &58.351 &13.859 &3.3647 &0.00051979 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &-1.571 &91.465 &91.632 &5.2741 &0.00099781 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &-0.9425 &72.425 &16.038 &4.1762 &0.00077447 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &-0.3142 &61.667 &9.8067 &3.5559 &0.0041261 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &0.3142 &46.863 &8.4076 &2.7023 &0.0025402 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &0.9425 &71.489 &15.125 &4.1223 &0.0062718 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &1.571 &29.558 &29.588 &1.7044 &0.0024421 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &2.199 &44.898 &10.716 &2.5889 &0.00098491 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.3 &2.827 &35.493 &5.7833 &2.0466 &9.0609e-05 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &-2.827 &63.958 &14.768 &3.688 &0.0016354 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &-2.199 &81.434 &37.199 &4.6957 &0.0039451 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &-0.9425 &54.852 &18.165 &3.1629 &0.002977 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &-0.3142 &92.25 &13.322 &5.3194 &0.0085319 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &0.3142 &51.015 &9.696 &2.9417 &0.0086483 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &0.9425 &68.98 &18.79 &3.9776 &0.0071007 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &2.199 &53.2 &15.571 &3.0677 &0.0026997 \\[0.05cm]
6.136 &0.4383 &1.352 &-0.1 &2.827 &34.039 &7.0027 &1.9628 &0.00085727 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &-2.827 &70.633 &18.125 &4.0729 &0.00081164 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &-2.199 &25.102 &12.798 &1.4475 &0.00024437 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &-0.9425 &77.394 &25.719 &4.4628 &0.010244 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &-0.3142 &60.007 &10.306 &3.4602 &0.0048227 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &0.3142 &75.607 &11.933 &4.3597 &0.0009242 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &0.9425 &111.67 &28.277 &6.4395 &0.0044222 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &2.199 &26.117 &11.95 &1.506 &0.0027502 \\[0.05cm]
6.136 &0.4383 &1.352 &0.1 &2.827 &55.737 &8.9523 &3.2139 &0.00092959 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &-2.827 &59.256 &10.349 &3.4169 &0.00049263 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &-2.199 &63.611 &31.963 &3.668 &0.0013274 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &-0.9425 &130.67 &64.256 &7.5347 &0.001684 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &-0.3142 &80.395 &13.243 &4.6358 &0.0025947 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &0.3142 &55.613 &9.2088 &3.2068 &0.00081461 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &0.9425 &36.826 &19.143 &2.1235 &0.0010293 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &2.199 &34.496 &18.239 &1.9891 &0.0032869 \\[0.05cm]
6.136 &0.4383 &1.352 &0.3 &2.827 &45.628 &9.3339 &2.631 &0.0038513 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &-2.827 &58.148 &16.173 &3.353 &0.00070868 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &-2.199 &55.557 &30.555 &3.2036 &0.0069829 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &-0.9425 &176.37 &59.036 &10.17 &0.0001309 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &-0.3142 &58.204 &10.898 &3.3562 &0.001708 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &0.3142 &58.595 &11.207 &3.3788 &0.0026909 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &0.9425 &74.867 &33.561 &4.317 &0.0079575 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &2.199 &76.404 &28.987 &4.4057 &0.0017736 \\[0.05cm]
6.136 &0.4383 &1.352 &0.5 &2.827 &66.995 &12.477 &3.8631 &0.00025502 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &-2.827 &53.399 &11.01 &3.0791 &0.00035977 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &-2.199 &53.423 &16.777 &3.0805 &0.0023635 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &-0.9425 &95.285 &24.901 &5.4944 &0.002709 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &-0.3142 &78.641 &17.983 &4.5346 &0.0011055 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &0.3142 &61.882 &11.379 &3.5683 &0.0012878 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &0.9425 &58.701 &14.625 &3.3849 &0.001965 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &1.571 &123.2 &88.441 &7.1038 &0.00080446 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &2.199 &122.27 &29.631 &7.0503 &0.0082363 \\[0.05cm]
6.136 &0.4383 &1.352 &0.7 &2.827 &57.195 &11.06 &3.298 &0.00092885 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &-2.827 &64.521 &13.66 &3.7205 &0.0019742 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &-2.199 &28.942 &7.4639 &1.6689 &0.0012742 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &-1.571 &72.615 &13.706 &4.1872 &0.0006302 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &-0.9425 &59.2 &10.236 &3.4136 &0.00066223 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &-0.3142 &70.901 &18.825 &4.0884 &0.0015174 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &0.3142 &63.149 &10.359 &3.6414 &0.00037099 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &0.9425 &83.292 &14.351 &4.8028 &0.0024762 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &1.571 &50.21 &10.644 &2.8952 &6.5338e-06 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &2.199 &59.526 &13.389 &3.4325 &0.00024438 \\[0.05cm]
6.136 &0.4383 &1.352 &0.9 &2.827 &60.554 &13.545 &3.4917 &0.0015125 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &-2.827 &27.094 &4.9948 &1.5623 &0.00099095 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &-2.199 &18.986 &4.3608 &1.0948 &0.0020569 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &-1.571 &16.432 &3.4943 &0.94751 &0.0018375 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &-0.9425 &26.398 &7.4156 &1.5222 &0.00081514 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &-0.3142 &15.128 &4.3934 &0.8723 &0.00070949 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &0.3142 &29.958 &7.3068 &1.7275 &0.001402 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &0.9425 &20.75 &4.3525 &1.1965 &0.0015717 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &1.571 &18.865 &6.4634 &1.0878 &0.0013034 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &2.199 &24.125 &4.4544 &1.3911 &0.0011581 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.9 &2.827 &26.536 &5.0501 &1.5301 &0.0022866 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &-2.827 &28.191 &6.1608 &1.6256 &7.6585e-05 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &-2.199 &31.881 &6.9269 &1.8384 &0.0047133 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &-1.571 &44.505 &12.007 &2.5663 &0.0065893 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &-0.9425 &27.35 &6.1426 &1.5771 &0.0021669 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &-0.3142 &27.306 &7.0158 &1.5745 &0.0022674 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &0.3142 &57.168 &17.868 &3.2965 &0.0014064 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &0.9425 &32.625 &7.0191 &1.8813 &0.00030221 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &1.571 &34.376 &9.1924 &1.9822 &0.0017357 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &2.199 &25.357 &5.715 &1.4622 &0.00095782 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.7 &2.827 &19.173 &4.8472 &1.1055 &0.00036301 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &-2.827 &24.817 &4.619 &1.431 &0.00036793 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &-2.199 &34.115 &7.478 &1.9672 &0.0024287 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &-1.571 &62.888 &35.771 &3.6263 &0.0061871 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &-0.9425 &75.926 &20.809 &4.3781 &0.0046349 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &-0.3142 &68.588 &17.73 &3.955 &0.0012918 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &0.3142 &39.951 &8.1455 &2.3037 &0.0014338 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &0.9425 &46.541 &14.214 &2.6837 &0.0013942 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &1.571 &89.188 &43.455 &5.1428 &0.0027491 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &2.199 &36.876 &8.3995 &2.1264 &0.0029686 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.5 &2.827 &38.448 &6.3428 &2.217 &0.0015748 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &-2.827 &36.482 &6.4766 &2.1037 &0.0016306 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &-2.199 &48.08 &14.866 &2.7724 &0.0064998 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &-0.9425 &54.241 &15.805 &3.1277 &0.0024591 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &-0.3142 &53.645 &10.164 &3.0933 &0.00078323 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &0.3142 &63.481 &10.126 &3.6605 &0.0030192 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &0.9425 &82.42 &20.427 &4.7526 &0.00011662 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &2.199 &36.972 &11.234 &2.1319 &7.8902e-05 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.3 &2.827 &37.476 &6.6194 &2.161 &0.0038246 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &-2.827 &41.284 &8.3593 &2.3806 &0.00043042 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &-2.199 &43.5 &28.3 &2.5084 &0.0012934 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &-0.9425 &61.908 &28.318 &3.5698 &0.0017046 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &-0.3142 &67.281 &11.525 &3.8796 &0.006947 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &0.3142 &63.949 &9.6059 &3.6875 &0.0040672 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &0.9425 &73.027 &23.826 &4.2109 &0.001103 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &2.199 &47.624 &19.528 &2.7461 &0.005335 \\[0.05cm]
6.06 &0.4351 &1.392 &-0.1 &2.827 &39.817 &8.3843 &2.296 &0.00063043 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &-2.827 &46.375 &10.246 &2.6741 &0.00056258 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &-2.199 &64.687 &38.328 &3.73 &0.0039126 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &-0.9425 &39.619 &28.582 &2.2846 &0.001385 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &-0.3142 &70.439 &12.315 &4.0617 &0.0058904 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &0.3142 &64.882 &10.807 &3.7413 &0.0026334 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &0.9425 &72.315 &30.707 &4.1699 &0.0036404 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &2.199 &89.637 &41.707 &5.1687 &0.0051903 \\[0.05cm]
6.06 &0.4351 &1.392 &0.1 &2.827 &55.928 &10.964 &3.2249 &0.0013816 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &-2.827 &50.376 &15.018 &2.9048 &0.00046857 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &-0.9425 &35.056 &24.912 &2.0214 &0.0025688 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &-0.3142 &74.283 &12.613 &4.2834 &0.0013014 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &0.3142 &78.6 &12.622 &4.5323 &0.00086647 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &0.9425 &24.532 &24.537 &1.4146 &0.0020015 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &2.199 &39.911 &39.918 &2.3014 &0.0027928 \\[0.05cm]
6.06 &0.4351 &1.392 &0.3 &2.827 &43.765 &14.722 &2.5236 &0.00077572 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &-2.827 &42.134 &14.502 &2.4296 &0.0049871 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &-2.199 &104.7 &52.38 &6.0372 &0.0017033 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &-0.9425 &25.752 &25.754 &1.4849 &0.0014221 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &-0.3142 &82.431 &20.253 &4.7532 &7.5753e-05 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &0.3142 &54.777 &10.81 &3.1586 &0.0021396 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &2.199 &20.739 &20.741 &1.1959 &0.0016202 \\[0.05cm]
6.06 &0.4351 &1.392 &0.5 &2.827 &49.361 &15.094 &2.8463 &0.00020037 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &-2.827 &57.94 &14.911 &3.341 &0.00108 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &-2.199 &60.465 &35.316 &3.4866 &0.00063926 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &-0.9425 &45.86 &20.613 &2.6444 &0.0058145 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &-0.3142 &56.117 &10.749 &3.2359 &0.00058032 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &0.3142 &46.533 &9.1128 &2.6832 &0.0013717 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &0.9425 &57.96 &24.42 &3.3422 &0.0012971 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &2.199 &23.525 &14.479 &1.3565 &0.0048573 \\[0.05cm]
6.06 &0.4351 &1.392 &0.7 &2.827 &45.044 &14.506 &2.5974 &0.00055027 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &-2.827 &78.569 &21.002 &4.5305 &1.2241e-05 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &-2.199 &67.039 &14.023 &3.8656 &0.00038436 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &-1.571 &42.788 &12.061 &2.4673 &0.0038439 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &-0.9425 &61.13 &13.227 &3.525 &0.00055187 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &-0.3142 &54.713 &9.894 &3.1549 &6.2709e-05 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &0.3142 &42.935 &8.2033 &2.4758 &0.0010595 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &0.9425 &57.117 &10.77 &3.2935 &0.00044453 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &1.571 &81.627 &15.171 &4.7069 &0.0005694 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &2.199 &67.568 &14.859 &3.8962 &0.00069891 \\[0.05cm]
6.06 &0.4351 &1.392 &0.9 &2.827 &56.286 &18.396 &3.2456 &4.9737e-05 \\[0.05cm]
  \end{longtable}
 \end{center}
\begin{center}
 \begin{longtable}{ccccccccc}
  \caption{\label{T:xntabh}Differential cross sections for the large SOS spectrometer angle.} \\
  \hline
  \hline
$Q^2$ &$\epsilon$ &$W$ &$\cos{\cm{\theta}}$ &$\cm{\phi}$ &$d\sigma^{\gamma^{\ast}}$ &$\sigma_{stat}$ &$\sigma_{norm}$ &$\sigma_{sys}$ \\
(GeV$^2$) &none &(GeV) &none &(rad) &(nb/Sr) &(nb/Sr) &(nb/Sr) &(nb/Sr) \\
  \hline \\[0.05cm]
  \endfirsthead
$Q^2$ &$\epsilon$ &$W$ &$\cos{\cm{\theta}}$ &$\cm{\phi}$ &$d\sigma^{\gamma^{\ast}}$ &$\sigma_{stat}$ &$\sigma_{norm}$ &$\sigma_{sys}$ \\
(GeV$^2$) &none &(GeV) &none &(rad) &(nb/Sr) &(nb/Sr) &(nb/Sr) &(nb/Sr) \\
  \hline \\[0.05cm]
  \endhead
7.924 &0.226 &1.112 &-0.83 &-2.618 &3.3484 &3.3484 &0.19308 &0.00010623 \\[0.05cm]
7.924 &0.226 &1.112 &-0.83 &-1.571 &5.4915 &3.8833 &0.31666 &0.0015979 \\[0.05cm]
7.924 &0.226 &1.112 &-0.83 &0.5236 &3.6922 &3.6923 &0.2129 &0.0011096 \\[0.05cm]
7.924 &0.226 &1.112 &-0.5 &-2.618 &10.699 &6.1777 &0.61693 &0.00074719 \\[0.05cm]
7.924 &0.226 &1.112 &-0.5 &-1.571 &3.2228 &3.2229 &0.18584 &4.5554e-05 \\[0.05cm]
7.924 &0.226 &1.112 &-0.5 &0.5236 &13.981 &8.0726 &0.80618 &0.0011314 \\[0.05cm]
7.924 &0.226 &1.112 &-0.5 &2.618 &11.165 &6.4639 &0.64379 &0.00056412 \\[0.05cm]
7.924 &0.226 &1.112 &-0.17 &-2.618 &3.9838 &3.9839 &0.22972 &0.00011688 \\[0.05cm]
7.924 &0.226 &1.112 &-0.17 &-0.5236 &14.114 &8.1561 &0.81385 &0.0033646 \\[0.05cm]
7.924 &0.226 &1.112 &-0.17 &0.5236 &9.2801 &6.5675 &0.53512 &0.006684 \\[0.05cm]
7.924 &0.226 &1.112 &-0.17 &1.571 &8.0517 &5.7423 &0.46428 &0.00073698 \\[0.05cm]
7.924 &0.226 &1.112 &0.17 &-1.571 &29.068 &17.276 &1.6762 &9.6845e-05 \\[0.05cm]
7.924 &0.226 &1.112 &0.17 &-0.5236 &11.745 &8.306 &0.67726 &0.0066473 \\[0.05cm]
7.924 &0.226 &1.112 &0.17 &0.5236 &10.744 &7.6031 &0.61951 &0.0059359 \\[0.05cm]
7.924 &0.226 &1.112 &0.17 &1.571 &17.438 &14 &1.0055 &0.0021233 \\[0.05cm]
7.924 &0.226 &1.112 &0.17 &2.618 &5.0387 &5.0388 &0.29054 &9.8618e-05 \\[0.05cm]
7.924 &0.226 &1.112 &0.5 &1.571 &7.5515 &7.5516 &0.43544 &0.00011164 \\[0.05cm]
7.924 &0.226 &1.112 &0.83 &-2.618 &19.899 &11.516 &1.1475 &0.00039875 \\[0.05cm]
7.924 &0.226 &1.112 &0.83 &-1.571 &13.04 &9.5684 &0.75195 &0.00049368 \\[0.05cm]
7.924 &0.226 &1.112 &0.83 &-0.5236 &33.666 &19.686 &1.9413 &0.00072406 \\[0.05cm]
7.924 &0.226 &1.112 &0.83 &1.571 &31.087 &12.735 &1.7925 &0.0012712 \\[0.05cm]
7.924 &0.226 &1.112 &0.83 &2.618 &14.287 &10.109 &0.82383 &0.00029197 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.83 &-1.571 &5.5822 &3.9473 &0.32189 &0.00078598 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.83 &0.5236 &14.352 &7.177 &0.8276 &0.0044191 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.83 &1.571 &3.3882 &3.3882 &0.19537 &0.0012187 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.5 &-2.618 &3.5583 &3.5584 &0.20518 &0.00021463 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.5 &-0.5236 &13.325 &7.7613 &0.76836 &0.0011438 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.5 &0.5236 &11.604 &6.7036 &0.6691 &0.0018878 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.5 &1.571 &11.729 &5.8799 &0.67631 &0.0024756 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.5 &2.618 &20.478 &13.992 &1.1808 &0.00056653 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.17 &-2.618 &5.7896 &5.7897 &0.33384 &0.00024831 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.17 &-1.571 &6.1311 &4.3363 &0.35353 &0.0003024 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.17 &0.5236 &11.997 &6.9268 &0.69176 &0.0033311 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.17 &1.571 &2.8432 &2.8433 &0.16395 &0.00027171 \\[0.05cm]
7.848 &0.2251 &1.152 &-0.17 &2.618 &11.466 &8.1089 &0.66117 &0.00070455 \\[0.05cm]
7.848 &0.2251 &1.152 &0.17 &-2.618 &17.256 &17.256 &0.99501 &0.00045627 \\[0.05cm]
7.848 &0.2251 &1.152 &0.17 &-1.571 &11.854 &8.4505 &0.68352 &0.00056817 \\[0.05cm]
7.848 &0.2251 &1.152 &0.17 &-0.5236 &7.0744 &7.0746 &0.40793 &0.0036365 \\[0.05cm]
7.848 &0.2251 &1.152 &0.17 &0.5236 &13.156 &9.3031 &0.7586 &0.0016436 \\[0.05cm]
7.848 &0.2251 &1.152 &0.17 &1.571 &31.061 &23.185 &1.7911 &0.001302 \\[0.05cm]
7.848 &0.2251 &1.152 &0.17 &2.618 &46.375 &46.377 &2.6741 &0.0011277 \\[0.05cm]
7.848 &0.2251 &1.152 &0.5 &-2.618 &25.023 &25.024 &1.4429 &0.00032798 \\[0.05cm]
7.848 &0.2251 &1.152 &0.5 &-1.571 &18.112 &9.3318 &1.0444 &0.0015421 \\[0.05cm]
7.848 &0.2251 &1.152 &0.5 &-0.5236 &27.126 &14.499 &1.5641 &0.0013942 \\[0.05cm]
7.848 &0.2251 &1.152 &0.5 &0.5236 &4.7865 &4.7866 &0.276 &0.0020987 \\[0.05cm]
7.848 &0.2251 &1.152 &0.5 &1.571 &13.599 &6.8193 &0.78413 &0.00036218 \\[0.05cm]
7.848 &0.2251 &1.152 &0.5 &2.618 &8.9608 &8.961 &0.51671 &0.00011271 \\[0.05cm]
7.848 &0.2251 &1.152 &0.83 &-2.618 &4.2515 &4.2515 &0.24515 &6.6678e-05 \\[0.05cm]
7.848 &0.2251 &1.152 &0.83 &-1.571 &21.369 &8.8954 &1.2322 &0.00036208 \\[0.05cm]
7.848 &0.2251 &1.152 &0.83 &-0.5236 &26.808 &10.234 &1.5458 &0.00019723 \\[0.05cm]
7.848 &0.2251 &1.152 &0.83 &0.5236 &24.168 &9.8914 &1.3936 &0.00087457 \\[0.05cm]
7.848 &0.2251 &1.152 &0.83 &1.571 &18.85 &7.7104 &1.0869 &0.00078445 \\[0.05cm]
7.848 &0.2251 &1.152 &0.83 &2.618 &19.734 &9.8732 &1.1379 &0.00022235 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.83 &-2.618 &10.588 &5.2944 &0.61052 &0.00025 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.83 &-1.571 &6.4468 &3.7226 &0.37174 &0.00022793 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.83 &-0.5236 &18.323 &7.4821 &1.0566 &0.00067405 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.83 &0.5236 &9.8699 &5.7445 &0.56913 &0.0022665 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.83 &1.571 &15.672 &8.3535 &0.90368 &0.0034349 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.83 &2.618 &21.105 &12.104 &1.217 &0.00020002 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.5 &-2.618 &13.317 &9.4174 &0.76791 &0.00039665 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.5 &-1.571 &23.545 &9.755 &1.3577 &0.0040139 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.5 &-0.5236 &19.908 &10.881 &1.148 &0.0015097 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.5 &0.5236 &18.551 &8.3046 &1.0697 &0.001413 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.5 &1.571 &13.843 &5.6531 &0.79824 &0.00029943 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.5 &2.618 &6.7048 &6.7051 &0.38662 &0.0018433 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.17 &-2.618 &22.378 &22.38 &1.2904 &0.0013837 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.17 &-1.571 &35.025 &16.933 &2.0197 &0.0023542 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.17 &-0.5236 &37.71 &13.371 &2.1745 &0.0045816 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.17 &0.5236 &35.196 &12.476 &2.0295 &0.0041438 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.17 &1.571 &14.925 &9.6109 &0.8606 &0.0022022 \\[0.05cm]
7.772 &0.2236 &1.192 &-0.17 &2.618 &20.829 &20.831 &1.201 &0.0010567 \\[0.05cm]
7.772 &0.2236 &1.192 &0.17 &-1.571 &23.071 &10.327 &1.3304 &0.00029619 \\[0.05cm]
7.772 &0.2236 &1.192 &0.17 &-0.5236 &52.05 &17.433 &3.0014 &0.0088928 \\[0.05cm]
7.772 &0.2236 &1.192 &0.17 &0.5236 &32.443 &13.276 &1.8708 &0.0050126 \\[0.05cm]
7.772 &0.2236 &1.192 &0.17 &1.571 &48.212 &23.968 &2.78 &0.0015804 \\[0.05cm]
7.772 &0.2236 &1.192 &0.5 &-2.618 &36.459 &25.875 &2.1023 &0.00098698 \\[0.05cm]
7.772 &0.2236 &1.192 &0.5 &-1.571 &66.02 &20.128 &3.8069 &0.00082584 \\[0.05cm]
7.772 &0.2236 &1.192 &0.5 &-0.5236 &46.419 &14.755 &2.6767 &0.00043443 \\[0.05cm]
7.772 &0.2236 &1.192 &0.5 &0.5236 &36.208 &12.15 &2.0879 &0.00021891 \\[0.05cm]
7.772 &0.2236 &1.192 &0.5 &1.571 &46.48 &16.6 &2.6802 &0.00021208 \\[0.05cm]
7.772 &0.2236 &1.192 &0.5 &2.618 &37.695 &26.656 &2.1736 &0.00097541 \\[0.05cm]
7.772 &0.2236 &1.192 &0.83 &-2.618 &56.981 &20.555 &3.2857 &0.00037297 \\[0.05cm]
7.772 &0.2236 &1.192 &0.83 &-1.571 &59.224 &15.915 &3.415 &0.00050917 \\[0.05cm]
7.772 &0.2236 &1.192 &0.83 &-0.5236 &32.197 &11.512 &1.8566 &0.00077946 \\[0.05cm]
7.772 &0.2236 &1.192 &0.83 &0.5236 &42.615 &13.725 &2.4573 &8.7906e-05 \\[0.05cm]
7.772 &0.2236 &1.192 &0.83 &1.571 &33.704 &11.178 &1.9435 &0.0005014 \\[0.05cm]
7.772 &0.2236 &1.192 &0.83 &2.618 &39.535 &16.161 &2.2797 &0.00071206 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.83 &-2.618 &18.075 &6.835 &1.0423 &0.00099205 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.83 &-1.571 &26.301 &7.486 &1.5166 &0.0010662 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.83 &-0.5236 &23.045 &7.6947 &1.3288 &0.0027881 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.83 &0.5236 &15.306 &9.1113 &0.88259 &0.0014566 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.83 &1.571 &11.892 &4.5166 &0.68573 &0.00053473 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.83 &2.618 &11.318 &5.6981 &0.65261 &0.00027116 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.5 &-2.618 &32.923 &23.288 &1.8984 &0.001383 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.5 &-1.571 &36.868 &11.136 &2.1259 &0.0028188 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.5 &-0.5236 &25.056 &9.5107 &1.4448 &0.0016132 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.5 &0.5236 &27.09 &9.5859 &1.5621 &0.0014495 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.5 &1.571 &29.065 &8.0958 &1.676 &0.0018555 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.5 &2.618 &15.217 &15.219 &0.87747 &1.6272e-05 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.17 &-1.571 &48.462 &18.728 &2.7945 &0.00047035 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.17 &-0.5236 &41.175 &13.731 &2.3743 &0.0010414 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.17 &0.5236 &43.714 &13.831 &2.5207 &0.0017335 \\[0.05cm]
7.692 &0.2222 &1.232 &-0.17 &1.571 &28.82 &13.242 &1.6618 &0.0038453 \\[0.05cm]
7.692 &0.2222 &1.232 &0.17 &-1.571 &50.048 &15.261 &2.8859 &0.0037811 \\[0.05cm]
7.692 &0.2222 &1.232 &0.17 &-0.5236 &21.716 &9.7903 &1.2522 &0.0055099 \\[0.05cm]
7.692 &0.2222 &1.232 &0.17 &0.5236 &31.125 &11.01 &1.7948 &0.011913 \\[0.05cm]
7.692 &0.2222 &1.232 &0.17 &1.571 &46.034 &19.788 &2.6545 &0.00074094 \\[0.05cm]
7.692 &0.2222 &1.232 &0.5 &-1.571 &42.301 &12.211 &2.4392 &9.4421e-05 \\[0.05cm]
7.692 &0.2222 &1.232 &0.5 &-0.5236 &28.358 &10.044 &1.6352 &0.00029008 \\[0.05cm]
7.692 &0.2222 &1.232 &0.5 &0.5236 &33.258 &11.473 &1.9178 &0.001228 \\[0.05cm]
7.692 &0.2222 &1.232 &0.5 &1.571 &59.134 &14.09 &3.4098 &0.00060575 \\[0.05cm]
7.692 &0.2222 &1.232 &0.83 &-2.618 &74.119 &33.194 &4.2739 &0.0010067 \\[0.05cm]
7.692 &0.2222 &1.232 &0.83 &-1.571 &30.912 &10.937 &1.7825 &0.001246 \\[0.05cm]
7.692 &0.2222 &1.232 &0.83 &-0.5236 &35.037 &16.12 &2.0204 &0.00044669 \\[0.05cm]
7.692 &0.2222 &1.232 &0.83 &0.5236 &50.212 &17.768 &2.8954 &0.0013599 \\[0.05cm]
7.692 &0.2222 &1.232 &0.83 &1.571 &59.388 &14.864 &3.4245 &0.0023799 \\[0.05cm]
7.692 &0.2222 &1.232 &0.83 &2.618 &14.303 &14.303 &0.82473 &0.00056046 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.83 &-2.618 &6.1055 &4.3174 &0.35206 &0.0010094 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.83 &-1.571 &13.135 &4.3991 &0.7574 &0.0013284 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.83 &-0.5236 &10.863 &4.8621 &0.6264 &0.0016022 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.83 &0.5236 &16.816 &7.5752 &0.96965 &0.00059702 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.83 &1.571 &16.737 &7.5946 &0.96508 &0.00073419 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.83 &2.618 &15.399 &8.3516 &0.88793 &0.0027862 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.5 &-2.618 &64.127 &64.162 &3.6977 &0.0059964 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.5 &-1.571 &38.573 &11.234 &2.2242 &0.00015797 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.5 &-0.5236 &18.207 &8.2 &1.0499 &0.0021686 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.5 &0.5236 &16.931 &7.5782 &0.97627 &0.003093 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.5 &1.571 &13.059 &4.9433 &0.753 &0.0022036 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.17 &-1.571 &40.359 &18.137 &2.3272 &0.0071377 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.17 &-0.5236 &45.58 &15.882 &2.6283 &0.0032173 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.17 &0.5236 &37.514 &12.507 &2.1632 &0.003268 \\[0.05cm]
7.608 &0.2211 &1.272 &-0.17 &1.571 &50.139 &15.899 &2.8912 &0.0040855 \\[0.05cm]
7.608 &0.2211 &1.272 &0.17 &-1.571 &50.695 &22.772 &2.9232 &0.0006272 \\[0.05cm]
7.608 &0.2211 &1.272 &0.17 &-0.5236 &37.782 &12.572 &2.1786 &0.0061952 \\[0.05cm]
7.608 &0.2211 &1.272 &0.17 &0.5236 &28.858 &9.6214 &1.664 &0.0048314 \\[0.05cm]
7.608 &0.2211 &1.272 &0.17 &1.571 &59.039 &21.901 &3.4043 &0.001555 \\[0.05cm]
7.608 &0.2211 &1.272 &0.5 &-1.571 &59.491 &18.843 &3.4304 &0.0045487 \\[0.05cm]
7.608 &0.2211 &1.272 &0.5 &-0.5236 &63.659 &17.737 &3.6707 &0.0028443 \\[0.05cm]
7.608 &0.2211 &1.272 &0.5 &0.5236 &55.127 &16.006 &3.1788 &0.0017551 \\[0.05cm]
7.608 &0.2211 &1.272 &0.5 &1.571 &64.049 &18.516 &3.6933 &0.00067222 \\[0.05cm]
7.608 &0.2211 &1.272 &0.83 &-2.618 &76.605 &76.61 &4.4173 &0.0036636 \\[0.05cm]
7.608 &0.2211 &1.272 &0.83 &-1.571 &6.0136 &6.0137 &0.34676 &0.0018603 \\[0.05cm]
7.608 &0.2211 &1.272 &0.83 &-0.5236 &35.986 &25.447 &2.075 &0.0013104 \\[0.05cm]
7.608 &0.2211 &1.272 &0.83 &1.571 &23.136 &11.569 &1.3341 &0.0010563 \\[0.05cm]
7.608 &0.2211 &1.272 &0.83 &2.618 &219.25 &219.26 &12.642 &0.0047868 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.83 &-2.618 &29.682 &14.356 &1.7115 &0.00726 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.83 &-1.571 &13.466 &5.3038 &0.77649 &0.0010701 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.83 &-0.5236 &8.3789 &4.1921 &0.48315 &0.001944 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.83 &0.5236 &10.684 &4.7877 &0.61606 &0.00090089 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.83 &1.571 &5.8716 &3.691 &0.33857 &0.00039011 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.83 &2.618 &16.374 &12.639 &0.94419 &0.0008161 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.5 &-1.571 &12.955 &5.2974 &0.74705 &0.0007746 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.5 &-0.5236 &30.488 &10.173 &1.758 &0.0014196 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.5 &0.5236 &22.909 &8.6618 &1.321 &0.002065 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.5 &1.571 &35.839 &10.387 &2.0666 &0.0032254 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.17 &-1.571 &34.861 &20.245 &2.0102 &0.00093936 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.17 &-0.5236 &26.975 &10.203 &1.5555 &0.0027568 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.17 &0.5236 &50.027 &13.925 &2.8847 &0.0042744 \\[0.05cm]
7.524 &0.2195 &1.312 &-0.17 &1.571 &22.386 &15.939 &1.2908 &0.0020131 \\[0.05cm]
7.524 &0.2195 &1.312 &0.17 &-0.5236 &62.894 &14.168 &3.6266 &0.0014433 \\[0.05cm]
7.524 &0.2195 &1.312 &0.17 &0.5236 &55.054 &13.447 &3.1745 &0.0044101 \\[0.05cm]
7.524 &0.2195 &1.312 &0.17 &1.571 &36.074 &36.077 &2.0801 &0.0017027 \\[0.05cm]
7.524 &0.2195 &1.312 &0.5 &-1.571 &36.713 &36.716 &2.117 &0.0031112 \\[0.05cm]
7.524 &0.2195 &1.312 &0.5 &-0.5236 &53.444 &24.076 &3.0817 &0.0020677 \\[0.05cm]
7.524 &0.2195 &1.312 &0.5 &0.5236 &32.794 &16.399 &1.891 &0.00010868 \\[0.05cm]
7.524 &0.2195 &1.312 &0.83 &0.5236 &120.72 &120.73 &6.9611 &0.0097336 \\[0.05cm]
7.524 &0.2195 &1.312 &0.83 &1.571 &18.23 &18.23 &1.0512 &0.00081793 \\[0.05cm]
7.436 &0.218 &1.352 &-0.83 &-2.618 &45.851 &38.273 &2.6439 &0.00063508 \\[0.05cm]
7.436 &0.218 &1.352 &-0.83 &-1.571 &19.676 &7.0949 &1.1346 &0.0010904 \\[0.05cm]
7.436 &0.218 &1.352 &-0.83 &-0.5236 &8.9881 &4.526 &0.51828 &0.0010801 \\[0.05cm]
7.436 &0.218 &1.352 &-0.83 &0.5236 &13.963 &5.2791 &0.80512 &0.0013711 \\[0.05cm]
7.436 &0.218 &1.352 &-0.83 &1.571 &10.901 &3.8548 &0.62858 &0.00072283 \\[0.05cm]
7.436 &0.218 &1.352 &-0.5 &-1.571 &35.792 &12.34 &2.0639 &0.0043071 \\[0.05cm]
7.436 &0.218 &1.352 &-0.5 &-0.5236 &36.072 &10.884 &2.08 &0.00082762 \\[0.05cm]
7.436 &0.218 &1.352 &-0.5 &0.5236 &24.146 &9.1564 &1.3923 &0.0044554 \\[0.05cm]
7.436 &0.218 &1.352 &-0.5 &1.571 &21.21 &7.5009 &1.223 &0.0016787 \\[0.05cm]
7.436 &0.218 &1.352 &-0.17 &-0.5236 &42.842 &12.422 &2.4704 &0.0020007 \\[0.05cm]
7.436 &0.218 &1.352 &-0.17 &0.5236 &36.447 &12.128 &2.1016 &0.0036234 \\[0.05cm]
7.436 &0.218 &1.352 &0.17 &-0.5236 &34.104 &11.404 &1.9665 &0.0048352 \\[0.05cm]
7.436 &0.218 &1.352 &0.17 &0.5236 &30.428 &10.822 &1.7546 &0.0030332 \\[0.05cm]
7.436 &0.218 &1.352 &0.5 &-0.5236 &144.8 &84.215 &8.3494 &0.0087912 \\[0.05cm]
7.436 &0.218 &1.352 &0.5 &0.5236 &35.331 &35.334 &2.0373 &0.0020981 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.83 &-1.571 &8.2185 &4.5833 &0.4739 &0.0010194 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.83 &-0.5236 &6.449 &4.8978 &0.37187 &0.00056916 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.83 &0.5236 &13.987 &8.8034 &0.80651 &0.0028548 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.83 &1.571 &9.7442 &3.6851 &0.56188 &0.00028599 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.5 &-1.571 &19.821 &8.8667 &1.1429 &0.00099428 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.5 &-0.5236 &23.102 &8.7385 &1.3322 &0.00077014 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.5 &0.5236 &29.477 &9.8296 &1.6997 &0.0018478 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.5 &1.571 &40.87 &16.562 &2.3567 &0.0012245 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.17 &-0.5236 &30.827 &10.911 &1.7775 &0.0018376 \\[0.05cm]
7.348 &0.2161 &1.392 &-0.17 &0.5236 &42.562 &12.302 &2.4543 &0.001583 \\[0.05cm]
7.348 &0.2161 &1.392 &0.17 &-0.5236 &57.24 &21.639 &3.3006 &0.0016017 \\[0.05cm]
7.348 &0.2161 &1.392 &0.17 &0.5236 &54.709 &20.685 &3.1546 &0.001308 \\[0.05cm]
  \end{longtable}
 \end{center}
\end{widetext}

